Improving Scene Text Recognition for Character-Level Long-Tailed Distribution

Despite the recent remarkable improvements in scene text recognition (STR), the majority of the studies focused mainly on the English language, which only includes few number of characters. However, STR models show a large performance degradation on languages with a numerous number of characters (e.g., Chinese and Korean), especially on characters that rarely appear due to the long-tailed distribution of characters in such languages. To address such an issue, we conducted an empirical analysis using synthetic datasets with different character-level distributions (e.g., balanced and long-tailed distributions). While increasing a substantial number of tail classes without considering the context helps the model to correctly recognize characters individually, training with such a synthetic dataset interferes the model with learning the contextual information (i.e., relation among characters), which is also important for predicting the whole word. Based on this motivation, we propose a novel Context-Aware and Free Experts Network (CAFE-Net) using two experts: 1) context-aware expert learns the contextual representation trained with a long-tailed dataset composed of common words used in everyday life and 2) context-free expert focuses on correctly predicting individual characters by utilizing a dataset with a balanced number of characters. By training two experts to focus on learning contextual and visual representations, respectively, we propose a novel confidence ensemble method to compensate the limitation of each expert. Through the experiments, we demonstrate that CAFE-Net improves the STR performance on languages containing numerous number of characters. Moreover, we show that CAFE-Net is easily applicable to various STR models.

==> table/experiment-ablation.tex <==
% Experiments - Ablation Study Table
\begin{table}[t!]
    \small
    \centering
    \begin{tabular}{@{}c@{}l|cc@{}c@{}|@{}c@{}}
        \toprule
        \multirowcell{1}{\multicolumn{1}{c}{\textbf{Lang.}}} & 
        \multirowcell{1}{\multicolumn{1}{c}{\textbf{Method}}} & \textbf{Real} & \textbf{Real$_{Easy}$} & \textbf{Real$_{Hard}$} &
        \textbf{WS$_{test}$} \\
        \midrule
        \multirowcell{3}{\textit{Kr}}
         & (A) Softmax
         & 77.43 & 77.87 & 61.25 & 86.37 \\
        
         & (B) +Ensemble 
         & 80.66 & 81.07 & 65.41 & 86.76 \\
        
         & (C) +External LM 
         & \textbf{81.35} & \textbf{81.75} & \textbf{66.68} & \textbf{88.93} \\
       \midrule
        \multirowcell{3}{\textit{Cn}}
         & (A) Softmax
         & 41.83 & 41.72 & 42.71 & 83.31 \\
        
         & (B) +Ensemble 
         & 45.77 & 46.04 & 43.66 & 83.46 \\
        
         & (C) +External LM 
         & \textbf{47.67} & \textbf{48.09} & \textbf{44.34} & \textbf{86.22} \\
        \bottomrule
    \end{tabular}
    \caption{Ablation study of TRBA + Ours. We demonstrate that the performance is enhanced by 1) employing the confidence ensemble of context-aware and -free experts and 2) incorporating an external language model into context-aware expert.}
    \vspace{-0.3cm}
    \label{Table:experiment-ablation}
\end{table}




















% \begin{table*}[t!]
%     \small
%     \centering
%     \begin{tabular}{@{}c@{}c@{}c@{}c|ccc|cc}
%         \toprule
%         \multirowcell{1}{\multicolumn{1}{c}{\textbf{Lang.}}} & 
%         \multirowcell{1}{\multicolumn{1}{c}{\textbf{Data}}} & 
%         \multirowcell{1}{\multicolumn{1}{c}{\textbf{Method}}} & 
%         \multirowcell{1}{\multicolumn{1}{c}{\textbf{Metric}}} & 
%         \textbf{Real} & \textbf{Real$_{Easy}$} & \textbf{Real$_{Hard}$} &
%         \textbf{WS$_{test}$} & \textbf{RS$_{test}$}\\
%         \midrule
%         \multirowcell{8}{\textit{Kr}}
%          & \multirowcell{2}{WS}
%          & \multirowcell{2}{Softmax} 
%          & Acc & 78.25 & 79.43 & 34.14 & 87.47 & 18.56 \\
%         %  && ED &  &  &  &  &  &  \\
%          &&& Char F1 & 0.34/0.77/0.87 & --/0.80/0.87 & 0.35/0.64/0.69 & 0.45/0.82/0.91 & 0.18/0.61/0.62 \\
%         \cmidrule(lr){2-9} 
%          & \multirowcell{2}{CS}
%          & \multirowcell{2}{Softmax}
%          & Acc & 75.77 & 76.10 & 63.51 & 73.65 & 73.32 \\
%         %  && ED & 0. & 0. & 0. & 0. & 0. & 0. \\
%          &&& Char F1 & 0.54/0.71/0.86 &  --/0.71/0.86 & 0.79/0.75/0.78 & 0.72/0.65/0.82 & 0.86/0.85/0.85 \\
%         \cmidrule(lr){2-9}
%          & \multirowcell{2}{CS}
%          & \multirowcell{2}{+Ensemble} 
%          & Acc &  &  &  &  &  \\
%         %  && ED &  &  &  &  &  &  \\
%          &&& Char F1 & // & --// & // & // & // \\
%         \cmidrule(lr){2-9}
%          & \multirowcell{2}{CS}
%          & \multirowcell{2}{+External LM} 
%          & Acc &  &  &  &  &  \\
%         %  && ED &  &  &  &  &  &  \\
%          &&& Char F1 & // & --// & // & // & // \\
%       \midrule
%         \multirowcell{8}{\textit{Cn}}
%          & \multirowcell{2}{WS}
%          & \multirowcell{2}{Softmax} 
%          & Acc & 39.19 & 42.99 & 9.25 & 83.23 & 9.05 \\
%         %  && ED & 0. & 0. & 0. & 0. & 0. & 0. \\
%          &&& Char F1 & 0.09/0.47/0.53 & --/0.51/0.55 & 0.10/0.47/0.49 & 0.15/0.77/0.89 & 0.07/0.56/0.53 \\
%         \cmidrule(lr){2-9} 
%          & \multirowcell{2}{CS}
%          & \multirowcell{2}{Softmax}
%          & Acc & 41.83 & 41.72 & 42.71 & 83.31 & 70.07 \\
%         %  && ED & 0. & 0. & 0. & 0. & 0. & 0. \\
%          &&& Char F1 & 0.48/0.54/0.57 & --/0.55/0.58 & 0.57/0.60/0.55 & 0.77/0.83/0.89 & 0.83/0.83/0.78 \\
%         \cmidrule(lr){2-9}
%          & \multirowcell{2}{CS}
%          & \multirowcell{2}{+Ensemble} 
%          & Acc &  &  &  &  &  \\
%         %  && ED &  &  &  &  &  &  \\
%          &&& Char F1 & // & --// & // & // & // \\
%         \cmidrule(lr){2-9}
%          & \multirowcell{2}{CS}
%          & \multirowcell{2}{+External LM} 
%          & Acc &  &  &  &  &  \\
%         %  && ED &  &  &  &  &  &  \\
%          &&& Char F1 & // & --// & // & // & // \\
%         \bottomrule
%     \end{tabular}
%     % \vspace{-0.2cm}
%     \caption{Ablation study of our method. Char F1 scores represent the scores of few/medium/many characters, respectively.}
%     % \vspace{-0.5cm}
%     \label{Table:experiment-ours}
% \end{table*}

==> table/experiment-dataset.tex <==
% Experiments - Dataset Table
\begin{table}[t!]
    \small
    \centering
    \begin{tabular}{@{}c@{}c@{}c@{}|c|c}
        \toprule
        \multirowcell{1}{\multicolumn{1}{c}{\textbf{Lang.}}} & 
        \multirowcell{1}{\multicolumn{1}{c}{\textbf{Data}}} & 
        \multirowcell{1}{\multicolumn{1}{c}{\textbf{Metric}}} & 
        \textbf{Real} & \textbf{Synth$_{test}$} \\
        \midrule
        \multirowcell{8}{\textit{Kr}}
         & \multirowcell{2}{WS} 
         & Acc & \textbf{78.25} & \textbf{87.47} \\
         && Char F1 & 0.34/0.77/0.87 & 0.18/0.61/0.62 \\
        \cmidrule(lr){2-5}
         & \multirowcell{2}{RS} 
         & Acc & 75.77 & 73.65 \\
         && Char F1 & 0.54/0.71/0.86 & \textbf{0.86}/\textbf{0.85}/\textbf{0.85} \\
        \cmidrule(lr){2-5}
         & \multirowcell{2}{CS} 
         & Acc & 77.43 & 86.37 \\
         && Char F1 & \textbf{0.66}/\textbf{0.79}/\textbf{0.88} & \textbf{0.86}/\textbf{0.85}/0.83 \\
        \midrule
        \multirowcell{8}{\textit{Cn}}
         & \multirowcell{2}{WS} 
         & Acc & 39.19 & 83.23 \\
         && Char F1 & 0.09/0.47/0.53 & 0.07/0.56/0.53 \\
        \cmidrule(lr){2-5}
         & \multirowcell{2}{RS} 
         & Acc & \textbf{42.26} & 67.95 \\
         && Char F1 & 0.40/0.49/\textbf{0.58} & 0.82/0.82/\textbf{0.82} \\
        \cmidrule(lr){2-5}
         & \multirowcell{2}{CS} 
         & Acc & 41.83 & \textbf{83.31} \\
         && Char F1 & \textbf{0.48}/\textbf{0.54}/0.57 & \textbf{0.83}/\textbf{0.83}/0.78 \\
        \bottomrule
    \end{tabular}
    \vspace{-0.2cm}
    \caption{Comparison of the performances trained with each synthetic dataset. Second column denotes the synthetic datasets used for training the model. Char F1 scores represent the scores of \textit{few} / \textit{medium} / \textit{many} characters, respectively.}
    \vspace{-0.5cm}
    \label{Table:experiment-dataset}
\end{table}


% Experiments - Dataset Table
% \begin{table}[t!]
%     \small
%     \centering
%     \begin{tabular}{c|cc|cc}
%         \toprule
%         \multirowcell{2}{\multicolumn{1}{c}{\textbf{Data}}} & \multicolumn{2}{c|}{\textit{Korean}} & \multicolumn{2}{c}{\textit{Chinese}} \\
%         & \textbf{Real} & \textbf{WS$_{test}$} & \textbf{Real} & \textbf{WS$_{test}$} \\
%         \midrule
%         WS & \textbf{78.25} & \textbf{87.47} & 39.19 & 83.23\\
%         RS & 75.77 & 73.65 & \textbf{42.26} & 67.95\\
%         CS & 77.43 & 86.37 & 41.83 & \textbf{83.31} \\
%         \bottomrule
%     \end{tabular}
%     \vspace{-0.2cm}
%     \caption{Comparison of the performances trained with each synthetic dataset. First column denotes the synthetic datasets used for training the model.}
%     \vspace{-0.5cm}
%     \label{Table:experiment-dataset}
% \end{table}

